Transformers Get Stable: An End-to-End Signal Propagation Theory for Language Models

In spite of their huge success, transformer models remain difficult to scale in depth. In this work, we develop a unified signal propagation theory and provide formulae that govern the moments of the forward and backward signal through the transformer model. Our framework can be used to understand and mitigate vanishing/exploding gradients, rank collapse, and instability associated with high attention scores. We also propose DeepScaleLM, an initialization and scaling scheme that conserves unit output/gradient moments throughout the model, enabling the training of very deep models with 1000 layers. We find that transformer models could be much deeper - our deep models with fewer parameters outperform shallow models in Language Modeling, Speech Translation, and Image Classification, across encoder-only, decoder-only and encoder-decoder variants, for both Pre-LN and Post-LN transformers, for multiple datasets and model sizes. These improvements also translate into improved performance on downstream Question Answering tasks and improved robustness for Image Classification.

==> fig/30B_final_grads.tex <==
% \begin{figure}[t]
% \begin{minipage}[b]{0.45\linewidth}
%     \begin{center}
%     \includegraphics[page=8]{fig/all_figs.pdf}
%     \caption{Gradient explodes backward for $64$-layer pre-LN, increasing hyperbolically with number of layers $N$, after $150$k training steps. Our theoretical models still hold - the model never escapes the regime it is initialized in.}
%     \label{fig:var_bck_30B_explode}
%     \end{center}
% \end{minipage}\hfill
% \begin{minipage}[b]{0.45\linewidth}
%     \begin{center}
%     \includegraphics[page=9]{fig/all_figs.pdf}
%     \caption{Linear growth in the forward pass for a $48$-layer $1024$-d PreLN model after training for $100$k steps. Our theoretical models still hold well.}
%     \label{fig:var_fwd_48_explode}
%     \end{center}
% \end{minipage}
% \end{figure}


==> sections/limitations.tex <==
\section{Limitations}

While our method specifically targets very deep models, and may directly benefit Large Language Models (LLMs) with billions of parameters, we could not test larger model sizes due to compute limitations. Our proposed scaling scheme, $\beta^2=\frac{2}{N}$ may not be optimal in cases where higher stability is required or where less stability is acceptable -- the optimal choice for $\beta^2=\frac{k}{N^\alpha}$ may vary across applications. Furthermore, while we observed our theoretical derivations remain approximately correct after $50$k training steps, the agreement does decrease as training progresses from initialization.
